Symbolic Models and Control of Discrete-Time Piecewise Affine Systems: An Approximate Simulation Approach

Symbolic models have been recently used as a sound mathematical formalism for the formal verification and control design of purely continuous and hybrid systems. In this paper we propose a sequence of symbolic models that approximates a discrete-time Piecewise Affine (PWA) system in the sense of approximate simulation and converges to the PWA system in the so-called simulation metric. Symbolic control design is then addressed with specifications expressed in terms of non-deterministic finite automata. A sequence of symbolic control strategies is derived which converges, in the sense of simulation metric, to the maximal controller solving the given specification on the PWA system.

==> stackrel.tex <==
%%
%% This is file `stackrel.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% stackrel.dtx  (with options: `package')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2006 by Heiko Oberdiek <oberdiek@uni-freiburg.de>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.3 of this license or (at your option) any later
%% version. The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of
%% LaTeX version 2005/12/01 or later.
%% 
%% This work has the LPPL maintenance status "maintained".
%% 
%% This Current Maintainer of this work is Heiko Oberdiek.
%% 
%% This work consists of the main source file stackrel.dtx
%% and the derived files
%%    stackrel.sty, stackrel.pdf, stackrel.ins, stackrel.drv.
%% 
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{stackrel}
  [2006/12/02 v1.0 Adding subscript option to stackrel (HO)]
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname unexpanded\endcsname\relax
  \newcommand*{\stack@relbin}[3][]{%
    \mathop{#3}\limits
    \toks@{#1}%
    \edef\reserved@a{\the\toks@}%
    \ifx\reserved@a\@empty\else_{#1}\fi
    \toks@{#2}%
    \edef\reserved@a{\the\toks@}%
    \ifx\reserved@a\@empty\else^{#2}\fi
    \egroup
  }%
\else
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname pdfstrcmp\endcsname\relax
    \newcommand*{\stack@relbin}[3][]{%
      \mathop{#3}\limits
      \edef\reserved@a{\unexpanded{#1}}%
      \ifx\reserved@a\@empty\else_{#1}\fi
      \edef\reserved@a{\unexpanded{#2}}%
      \ifx\reserved@a\@empty\else^{#2}\fi
      \egroup
    }%
  \else
    \newcommand*{\stack@relbin}[3][]{%
      \mathop{#3}\limits
      \ifcase\pdfstrcmp{\detokenize{#1}}{}\else_{#1}\fi
      \ifcase\pdfstrcmp{\detokenize{#2}}{}\else^{#2}\fi
      \egroup
    }%
  \fi
\fi
\renewcommand*{\stackrel}{%
  \mathrel\bgroup\stack@relbin
}
\newcommand*{\stackbin}{%
  \mathbin\bgroup\stack@relbin
}
\endinput
%%
%% End of file `stackrel.sty'.
